Privacy in Location Based Services: Primitives Toward the Solution

Location based services (LBS) are one of the most promising and innovative directions of convergence technologies resulting of emergence of several fields including database systems, mobile communication, Internet technology, and positioning systems. Although being initiated as early as middle of 1990's, it is only recently that the LBS received a systematic profound research interest due to its commercial and technological impact. As the LBS is related to the user's location which can be used to trace the user's activities, a strong privacy concern has been raised. To preserve the user's location, several intelligent works have been introduced though many challenges are still awaiting solutions. This paper introduces a survey on LBS systems considering both localization technologies, model and architectures guaranteeing privacy. We also overview cryptographic primitive to possibly use in preserving LBS's privacy followed by fruitful research directions basically concerned with the privacy issue.

==> Latex8.txt <==
========== file:  LATEX.TXT =======================

The following files contain the LaTeX macros necessary for you to format 
your paper based on the instructions/measurements in the INSTRUCT.TXT 
attachment in our standard author kit for 8.5 x 11-inch proceedings. 
The files appear in the following order:

latex8.sty -- the style file
latex8.tex -- the main macro set
latex8.bib -- the sample bibliography macros
latex8.bst -- the bibliography main macro set
latex8ps.txt -- this file, when printed out, will give you a sample 
of how your paper should look when it's finished. This file is in a 
separate attachment from the first four LaTeX files. Remember to save 
it as a .ps file and strip out any extraneous lines at the top of the 
file to enable successful printing.

Note that both current versions of LaTeX, 2e and 2.09, have the same 
macros -- refer to the start of the latex8.sty file for the opening 
statement for each. 


